Generative Modeling for Low Dimensional Speech Attributes with Neural Spline Flows

Despite recent advances in generative modeling for text-to-speech synthesis, these models do not yet have the same fine-grained adjustability of pitch-conditioned deterministic models such as FastPitch and FastSpeech2. Pitch information is not only low-dimensional, but also discontinuous, making it particularly difficult to model in a generative setting. Our work explores several techniques for handling the aforementioned issues in the context of Normalizing Flow models. We also find this problem to be very well suited for Neural Spline flows, which is a highly expressive alternative to the more common affine-coupling mechanism in Normalizing Flows.

==> plot_sigma_sweep.tex <==
\pgfplotstableread[col sep=comma]{ftp_mfa_mcd.csv}\mfamcdraw
\pgfplotstablesort[sort key=model, sort cmp=int >]{\mfamcd}{\mfamcdraw}

\begin{figure}
    \centering
    \begin{tikzpicture}[]
      \begin{axis}[
        height=3.75cm,
        width=0.95\linewidth,
          xlabel= Iteration,
          ylabel= {MCD-DTW},
          ylabel near ticks,
          xlabel near ticks,
          xlabel style= {font=\small},
          ylabel style={font=\small},
          legend style={font=\tiny},
          yticklabel style = {font=\tiny},
          xticklabel style = {font=\tiny},
          ymode=log,
          log basis y={10},
          legend columns=1,
          legend entries={RADTTS LJSpeech Alignment, RADTTS LJSpeech MFA, RADTTS LibriTTS Alignment, RADTTS LibriTTS MFA}
        ]
        \addplot [line width=0.3mm, color=glaucous] table [x=model, y=mel_cepstrum_mcd,col sep=comma] {\betabinomialmcd};
        
        \addplot [line width=0.3mm, color=lava] table [x=model, y=mel_cepstrum_mcd, col sep=comma] {\mfamcd};
        
        \addplot [line width=0.3mm, color=forestgreen] table [x=model, y=mel_cepstrum_mcd,col sep=comma] {\libribetabinomialmcd};
        
        \addplot [line width=0.3mm, color=chromeyellow] table [x=model, y=mel_cepstrum_mcd, col sep=comma] {\librimfamcd};
      \end{axis}
    \end{tikzpicture}
    \caption{MCD-DTW metric curves demonstrating converging speed of various models, computed on validation data.}
    \label{fig:mcd_dtw}
    \vspace{-1em}
\end{figure}
